Technology and jobs: A systematic literature review

Does technological change destroy or create jobs? New technologies may replace human workers, but can simultaneously create jobs if workers are needed to use these technologies or if new economic activities emerge. Furthermore, technology-driven productivity growth may increase disposable income, stimulating a demand-induced expansion of employment. To synthesize the existing knowledge on this question, we systematically review the empirical literature on the past four decades of technological change and its impact on employment, distinguishing between five broad technology categories (ICT, Robots, Innovation, TFP-style, Other). Overall, we find across studies that the labor-displacing effect of technology appears to be more than offset by compensating mechanisms that create or reinstate labor. This holds for most types of technology, suggesting that previous anxieties over widespread technology-driven unemployment lack an empirical base, at least so far. Nevertheless, low-skill, production, and manufacturing workers have been adversely affected by technological change, and effective up- and reskilling strategies should remain at the forefront of policy making along with targeted social support systems.

==> inputs/stats_byeffect.tex <==
            & replacement&reinstatement&  real income&     overlap\\
\midrule
share       &        0.81&        0.62&        0.26&        0.59\\
\#          &         103&          79&          33&          75\\


==> inputs/stats_byeffect_short.tex <==
 \textbf{Panel A: Effect}  & Replacement&Reinstatement&  Real income&     Overlap\\
\midrule
share       &        0.81&        0.62&        0.26&        0.59\\
\#          &         103&          79&          33&          75\\


==> inputs/stats_byheterog.tex <==
            &         any&     replace&      reinst&     realinc&       total\\
\midrule
share       &        0.53&        0.58&        0.66&        0.55&        0.63\\
\#          &          67&          60&          52&          18&          56\\


==> inputs/stats_bylevel.tex <==
            &       macro&        meso&       micro&    regional&     overlap\\
\midrule
share       &        0.35&        0.32&        0.30&        0.12&        0.09\\
\#          &          45&          41&          38&          15&          12\\


==> inputs/stats_bylevel_short.tex <==
\textbf{Panel C: Level of analysis} &       Macro&        Meso&       Micro&    Regional&     Overlap\\
\midrule
share       &        0.35&        0.32&        0.30&        0.12&        0.09\\
\#          &          45&          41&          38&          15&          12\\


==> inputs/stats_bytech.tex <==
            &         ICT&       Robots&  Innovation&    TFP-style&       Other&     Overlap\\
\midrule
share       &        0.35&        0.13&        0.13&        0.14&        0.30&        0.06\\
\#          &          45&          17&          17&          18&          38&           8\\


==> inputs/stats_bytech_short.tex <==
 \textbf{Panel B: Technology} &         ICT&       Robots&  Innovation&    TFP-style&       Other&     Overlap\\
\midrule
share       &        0.35&        0.13&        0.13&        0.14&        0.30&        0.06\\
\#          &          45&          17&          17&          18&          38&           8\\

==> inputs/stats_effect_byheterogeneity.tex <==
\multicolumn{1}{l}{\textbf{\emph{Any effect}}} & \multicolumn{6}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.17&        0.13&        0.20&        0.24&        0.09&        0.07\\
\#          &          21&          17&          26&          30&          11&           9\\
\multicolumn{1}{l}{\textbf{\emph{Replacement}}} & \multicolumn{6}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.16&        0.17&        0.25&        0.28&        0.11&        0.05\\
\#          &          16&          17&          26&          29&          11&           5\\
\multicolumn{1}{l}{\textbf{\emph{Reinstatement}}} & \multicolumn{6}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.25&        0.16&        0.25&        0.30&        0.09&        0.09\\
\#          &          20&          13&          20&          24&           7&           7\\
\multicolumn{1}{l}{\textbf{\emph{Real income}}} & \multicolumn{6}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.24&        0.12&        0.21&        0.21&        0.09&        0.03\\
\#          &           8&           4&           7&           7&           3&           1\\
\multicolumn{1}{l}{\textbf{\emph{Net employment}}} & \multicolumn{6}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.22&        0.18&        0.24&        0.26&        0.10&        0.10\\
\#          &          20&          16&          21&          23&           9&           9\\


==> inputs/stats_effect_bymethod.tex <==
\multicolumn{1}{l}{\textbf{\emph{Any effect}}} & \multicolumn{3}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.14&        0.80&        0.06\\
\#          &          18&         102&           7\\
\multicolumn{1}{l}{\textbf{\emph{Replacement}}} & \multicolumn{3}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.15&        0.83&        0.03\\
\#          &          15&          85&           3\\
\multicolumn{1}{l}{\textbf{\emph{Reinstatement}}} & \multicolumn{3}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.16&        0.80&        0.04\\
\#          &          13&          63&           3\\
\multicolumn{1}{l}{\textbf{\emph{Real income}}} & \multicolumn{3}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.12&        0.85&        0.03\\
\#          &           4&          28&           1\\
\multicolumn{1}{l}{\textbf{\emph{Net employment}}} & \multicolumn{3}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.15&        0.81&        0.04\\
\#          &          13&          72&           4\\


==> inputs/stats_effect_bymethod_short.tex <==
\textbf{Panel D: Methodology} & \multicolumn{1}{c}{Descriptive}&\multicolumn{1}{c}{Regression}&\multicolumn{1}{c}{Simulation}\\ \midrule
share       &        0.14&        0.80&        0.06\\
\#          &          18&         102&           7\\


==> inputs/stats_grealinc_byfind.tex <==
            &productivity&      prices&      income&      output&       other\\
\midrule
share       &        0.68&        0.09&        0.29&        0.18&        0.06\\
\#          &          23&           3&          10&           6&           2\\


==> inputs/stats_grealinc_byfind_incl_nanr.tex <==
            &productivity&      prices&      income&      output&       other&        na/nr\\
\midrule
share       &        0.18&        0.02&        0.08&        0.05&        0.02&        0.73\\
\#          &          23&           3&          10&           6&           2&          93\\


==> inputs/stats_level_byfind_realinc.tex <==
\multicolumn{1}{l}{\textbf{\emph{macro}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.75&        0.08&        0.08&        0.08\\
\#          &           9&           1&           1&           1\\
\multicolumn{1}{l}{\textbf{\emph{meso}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.87&       0&        0.07&        0.07\\
\#          &          13&           0&           1&           1\\
\multicolumn{1}{l}{\textbf{\emph{micro}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.17&        0.50&       0&        0.33\\
\#          &           1&           3&           0&           2\\
\multicolumn{1}{l}{\textbf{\emph{regional}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.75&        0.25&       0&       0\\
\#          &           3&           1&           0&           0\\


==> inputs/stats_level_byfind_reinst.tex <==
\multicolumn{1}{l}{\textbf{\emph{macro}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.77&        0.12&        0.08&        0.04\\
\#          &          20&           3&           2&           1\\
\multicolumn{1}{l}{\textbf{\emph{meso}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.93&        0.04&        0.04&       0\\
\#          &          25&           1&           1&           0\\
\multicolumn{1}{l}{\textbf{\emph{micro}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.68&        0.18&        0.14&       0\\
\#          &          15&           4&           3&           0\\
\multicolumn{1}{l}{\textbf{\emph{regional}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.91&       0&       0&        0.09\\
\#          &          10&           0&           0&           1\\


==> inputs/stats_level_byfind_replace.tex <==
\multicolumn{1}{l}{\textbf{\emph{macro}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.69&        0.11&        0.09&        0.11\\
\#          &          24&           4&           3&           4\\
\multicolumn{1}{l}{\textbf{\emph{meso}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.81&        0.11&        0.03&        0.06\\
\#          &          29&           4&           1&           2\\
\multicolumn{1}{l}{\textbf{\emph{micro}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.48&        0.23&        0.03&        0.26\\
\#          &          15&           7&           1&           8\\
\multicolumn{1}{l}{\textbf{\emph{regional}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.73&       0&       0&        0.27\\
\#          &           8&           0&           0&           3\\


==> inputs/stats_level_byfind_total.tex <==
\multicolumn{1}{l}{\textbf{\emph{macro}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.18&        0.33&        0.18&        0.30\\
\#          &           6&          11&           6&          10\\
\multicolumn{1}{l}{\textbf{\emph{meso}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.22&        0.37&        0.26&        0.15\\
\#          &           6&          10&           7&           4\\
\multicolumn{1}{l}{\textbf{\emph{micro}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.46&        0.33&        0.08&        0.13\\
\#          &          11&           8&           2&           3\\
\multicolumn{1}{l}{\textbf{\emph{regional}}} & \multicolumn{4}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.42&        0.42&        0.08&        0.08\\
\#          &           5&           5&           1&           1\\


==> inputs/stats_realinc_byfind.tex <==
            &     support&     depends&        weak&   no support\\
\midrule
share       &        0.70&        0.12&        0.06&        0.12\\
\#          &          23&           4&           2&           4\\


==> inputs/stats_realinc_byfind_incl_nanr.tex <==
            &     support&     depends&        weak&   no support&        na/nr\\
\midrule
share       &        0.18&        0.03&        0.02&        0.03&        0.74\\
\#          &          23&           4&           2&           4&          94\\


==> inputs/stats_realinc_byheterog.tex <==
            &     support&     depends&        weak&   no support\\
\midrule
share       &        0.61&        0.75&        0.50&       0\\
\#          &          14&           3&           1&           0\\


==> inputs/stats_realinc_bylevel.tex <==
share       &        0.36&        0.45&        0.18&        0.12\\
\#          &          12&          15&           6&           4\\


==> inputs/stats_realinc_bytech.tex <==
share       &        0.36&        0.27&        0.06&        0.18&        0.15\\
\#          &          12&           9&           2&           6&           5\\


==> inputs/stats_reinst_byfind.tex <==
            &     support&     depends&        weak&   no support\\
\midrule
share       &        0.81&        0.09&        0.08&        0.03\\
\#          &          64&           7&           6&           2\\


==> inputs/stats_reinst_byfind_incl_nanr.tex <==
            &     support&     depends&        weak&   no support&        na/nr\\
\midrule
share       &        0.50&        0.06&        0.05&        0.02&        0.38\\
\#          &          64&           7&           6&           2&          48\\


==> inputs/stats_reinst_byheterog.tex <==
            &     support&     depends&        weak&   no support\\
\midrule
share       &        0.69&        0.71&        0.17&        1.00\\
\#          &          44&           5&           1&           2\\


==> inputs/stats_reinst_bylevel.tex <==
share       &        0.33&        0.34&        0.28&        0.14\\
\#          &          26&          27&          22&          11\\


==> inputs/stats_reinst_bytech.tex <==
share       &        0.38&        0.13&        0.18&        0.14&        0.28\\
\#          &          30&          10&          14&          11&          22\\


==> inputs/stats_replace_byfind.tex <==
            &     support&     depends&        weak&   no support\\
\midrule
share       &        0.67&        0.13&        0.05&        0.16\\
\#          &          69&          13&           5&          16\\


==> inputs/stats_replace_byfind_incl_nanr.tex <==
            &     support&     depends&        weak&   no support&        na/nr\\
\midrule
share       &        0.54&        0.10&        0.04&        0.13&        0.19\\
\#          &          69&          13&           5&          16&          24\\


==> inputs/stats_replace_byheterog.tex <==
            &     support&     depends&        weak&   no support\\
\midrule
share       &        0.55&        0.77&        0.40&        0.63\\
\#          &          38&          10&           2&          10\\


==> inputs/stats_replace_bylevel.tex <==
share       &        0.34&        0.35&        0.30&        0.11\\
\#          &          35&          36&          31&          11\\


==> inputs/stats_replace_bytech.tex <==
share       &        0.36&        0.15&        0.12&        0.17&        0.29\\
\#          &          37&          15&          12&          17&          30\\


==> inputs/stats_tech_byfind_realinc.tex <==
\multicolumn{1}{l}{\textbf{\emph{ICT}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.36&        0.83&       0&       0&        0.17\\
\#          &          12&          10&           0&           0&           2\\
\multicolumn{1}{l}{\textbf{\emph{Robots}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.27&        0.67&        0.22&        0.11&       0\\
\#          &           9&           6&           2&           1&           0\\
\multicolumn{1}{l}{\textbf{\emph{Innovation}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.06&        0.50&        0.50&       0&       0\\
\#          &           2&           1&           1&           0&           0\\
\multicolumn{1}{l}{\textbf{\emph{TFP-style}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.18&        0.83&       0&       0&        0.17\\
\#          &           6&           5&           0&           0&           1\\
\multicolumn{1}{l}{\textbf{\emph{Other}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.15&        0.40&        0.20&        0.20&        0.20\\
\#          &           5&           2&           1&           1&           1\\


==> inputs/stats_tech_byfind_reinst.tex <==
\multicolumn{1}{l}{\textbf{\emph{ICT}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.38&        0.77&        0.07&        0.13&        0.03\\
\#          &          30&          23&           2&           4&           1\\
\multicolumn{1}{l}{\textbf{\emph{Robots}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.13&        0.90&       0&       0&        0.10\\
\#          &          10&           9&           0&           0&           1\\
\multicolumn{1}{l}{\textbf{\emph{Innovation}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.18&        0.57&        0.29&        0.14&       0\\
\#          &          14&           8&           4&           2&           0\\
\multicolumn{1}{l}{\textbf{\emph{TFP-style}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.14&        0.91&        0.09&       0&       0\\
\#          &          11&          10&           1&           0&           0\\
\multicolumn{1}{l}{\textbf{\emph{Other}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.28&        0.91&        0.05&        0.05&       0\\
\#          &          22&          20&           1&           1&           0\\


==> inputs/stats_tech_byfind_replace.tex <==
\multicolumn{1}{l}{\textbf{\emph{ICT}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.36&        0.62&        0.08&        0.05&        0.24\\
\#          &          37&          23&           3&           2&           9\\
\multicolumn{1}{l}{\textbf{\emph{Robots}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.15&        0.87&       0&       0&        0.13\\
\#          &          15&          13&           0&           0&           2\\
\multicolumn{1}{l}{\textbf{\emph{Innovation}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.12&        0.25&        0.58&       0&        0.17\\
\#          &          12&           3&           7&           0&           2\\
\multicolumn{1}{l}{\textbf{\emph{TFP-style}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.17&        0.76&        0.12&        0.06&        0.06\\
\#          &          17&          13&           2&           1&           1\\
\multicolumn{1}{l}{\textbf{\emph{Other}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.29&        0.73&        0.10&        0.07&        0.10\\
\#          &          30&          22&           3&           2&           3\\


==> inputs/stats_tech_byfind_total.tex <==
\multicolumn{1}{l}{\textbf{\emph{ICT}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.29&        0.27&        0.42&        0.23&        0.08\\
\#          &          26&           7&          11&           6&           2\\
\multicolumn{1}{l}{\textbf{\emph{Robots}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.16&        0.36&        0.14&        0.29&        0.21\\
\#          &          14&           5&           2&           4&           3\\
\multicolumn{1}{l}{\textbf{\emph{Innovation}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.15&        0.46&        0.38&        0.15&       0\\
\#          &          13&           6&           5&           2&           0\\
\multicolumn{1}{l}{\textbf{\emph{TFP-style}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.15&        0.08&        0.38&        0.15&        0.38\\
\#          &          13&           1&           5&           2&           5\\
\multicolumn{1}{l}{\textbf{\emph{Other}}} & \multicolumn{5}{c}{} \\\cmidrule(l{4pt}r{4pt}){1-1}
share       &        0.33&        0.28&        0.41&        0.10&        0.21\\
\#          &          29&           8&          12&           3&           6\\


==> inputs/stats_total_byfind.tex <==
            &    positive&     depends&        weak&    negative\\
\midrule
share       &        0.29&        0.35&        0.18&        0.18\\
\#          &          26&          31&          16&          16\\


==> inputs/stats_total_byfind_incl_nanr.tex <==
            &    positive&     depends&        weak&    negative&        na/nr\\
\midrule
share       &        0.20&        0.24&        0.13&        0.13&        0.30\\
\#          &          26&          31&          16&          16&          38\\


==> inputs/stats_total_byheterog.tex <==
            &    positive&    negative&     depends&        weak\\
\midrule
share       &        0.65&        0.44&        0.74&        0.56\\
\#          &          17&           7&          23&           9\\


==> inputs/stats_total_bylevel.tex <==
share       &        0.37&        0.30&        0.27&        0.13\\
\#          &          33&          27&          24&          12\\


==> inputs/stats_total_bytech.tex <==
share       &        0.29&        0.16&        0.15&        0.15&        0.33\\
\#          &          26&          14&          13&          13&          29\\


==> inputs/studies1.tex <==
\begin{tabular}{ll*{8}{c}}
\toprule
\multicolumn{2}{c}{Studies} & \multicolumn{3}{c}{Categories} & \multicolumn{5}{c}{Findings for technology effects on} \\
\midrule
\multicolumn{1}{p{2em}}{\#} & Authors \& year & Technology & Level of  & Empirical & Net   & Replacement & Reinstatement & \multicolumn{2}{c}{Real income} \\
\cmidrule{9-10}      & \multicolumn{1}{c}{} & group & analysis & methods & employment & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & finding & type \\
\midrule
1     & \cite{acemoglu2019automation} & robots & meso  & regression & weak  & support & support & support & productivity \\
2     & \cite{acemoglu2020robots} & robots & regional & regression & negative & support & no support & support & productivity \\
3     & \cite{addison2000tech} & ICT   & micro & regression & negative & support & na/nr & na/nr & na/nr \\
4     & \cite{angelini2020wage} & TFP-style & meso  & descriptive & na/nr & support & support & na/nr & na/nr \\
5     & \cite{arntz2017} & other/indirect & micro & regression & negative & support & na/nr & na/nr & na/nr \\
6     & \cite{atasoy2016} & ICT   & micro & regression & positive & no support & na/nr & na/nr & na/nr \\
7     & \cite{atasoy2013broadband} & ICT   & regional & regression & positive & na/nr & support & na/nr & na/nr \\
8     & \cite{auberttarby2018} & ICT   & micro & regression & positive & no support & support & na/nr & na/nr \\
9     & \cite{autor2015trade} & ICT   & regional & regression & depends & support & support & na/nr & na/nr \\
10    & \cite{autor2013polar} & ICT   & regional & regression & na/nr & support & support & na/nr & na/nr \\
11    & \cite{autor1998computers} & ICT   & macro & regression & na/nr & weak  & weak  & na/nr & na/nr \\
12    & \cite{autor2002computers} & ICT   & meso  & descriptive & na/nr & support & na/nr & support & productivity \\
13    & \cite{autor2003skill} & ICT   & meso  & regression & na/nr & support & support & na/nr & na/nr \\
14    & \cite{autor2018lshare} & TFP-style & macro; & regression & negative & support & support & support & productivity; \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & meso  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & income \\
15    & \cite{autor2015there} & ICT   & macro & descriptive & weak  & support & support & support & productivity; \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & income \\
16    & \cite{baddeley2008structural} & ICT   & macro & regression & na/nr & support & support & support & productivity \\
17    & \cite{badescu2009impact} & ICT   & micro & regression & na/nr & na/nr & na/nr & no support & productivity \\
18    & \cite{balleer2012new} & other/indirect & macro & other & negative & na/nr & na/nr & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & (simulation) & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
19    & \cite{balsmeier2019time} & ICT   & micro & regression & positive & support & support & na/nr & na/nr \\
20    & \cite{baltagi2005skill} & TFP-style & macro & regression & na/nr & support & support & na/nr & na/nr \\
21    & \cite{behaghel2016it} & ICT   & regional & regression & weak  & no support & support & na/nr & na/nr \\
22    & \cite{berman1994changes} & ICT   & meso  & regression & weak  & support & support & support & income \\
23    & \cite{bessen2020autom} & TFP-style & meso  & regression & depends & support & support & support & productivity; \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & prices \\
24    & \cite{biagi2017ict} & ICT   & meso  & regression & na/nr & no support & na/nr & na/nr & na/nr \\
25    & \cite{blanas2019who} & ICT;  & meso  & regression & depends & support & support & support & income \\
      & \multicolumn{1}{l}{} & robots & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
26    & \cite{blien2021occup} & other/indirect & micro & regression & na/nr & support & na/nr & depends & income \\
27    & \cite{bloch2010technological} & TFP-style & meso  & regression & weak  & support & na/nr & na/nr & na/nr \\
28    & \cite{bogliacino2010inno} & innovation & meso  & regression & na/nr & depends & na/nr & na/nr & na/nr \\
29    & \cite{borjas2019} & robots & regional; & regression & na/nr & support & na/nr & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & meso  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
30    & \cite{borland2017robot} & ICT   & macro & descriptive & weak  & no support & depends & na/nr & na/nr \\
31    & \cite{boyle2002trade} & TFP-style & macro & regression & weak  & depends & support & support & productivity; \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & income \\
32    & \cite{breemersch2019polar} & ICT;  & meso  & regression & weak  & depends & weak  & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & other/indirect & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
33    & \cite{buyst2018polar} & other/indirect & macro; & descriptive & na/nr & support & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & meso  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
34    & \cite{calvino2018innovation} & innovation & micro & descriptive & positive & no support & support & na/nr & na/nr \\
35    & \cite{camina2020autom} & robots & micro & regression & positive & support & na/nr & depends & productivity \\
36    & \cite{capello2013inno} & innovation & regional & regression & depends & na/nr & support & na/nr & na/nr \\
37    & \cite{charalampidis2019} & ICT   & macro & other & weak  & na/nr & weak  & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & (simulation) & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
38    & \cite{chen2014total} & TFP-style & macro & regression & negative & support & na/nr & support & productivity \\
39    & \cite{chun2015it} & ICT   & micro & regression & na/nr & na/nr & na/nr & support & productivity \\
40    & \cite{cirillo2017tech} & innovation & meso  & regression & depends & support & support & support & output \\
41    & \cite{colombo2013ict} & ICT   & micro & regression & na/nr & na/nr & na/nr & no support & productivity \\
42    & \cite{compagnucci2019robotization} & robots & meso  & regression & negative & support & na/nr & weak  & prices; \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & income \\
43    & \cite{cozzarin2016inno} & innovation & micro & regression & na/nr & depends & na/nr & depends & productivity; \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & income \\
44    & \cite{dachs2017inno} & innovation & micro & regression & positive & support & support & na/nr & na/nr \\
45    & \cite{devries2020rise} & robots & meso  & regression & weak  & support & support & na/nr & na/nr \\
46    & \cite{dekle2020robot} & robots & meso  & regression & positive & no support & support & support & productivity \\
47    & \cite{dengler2018tech} & ICT   & micro & regression & na/nr & support & na/nr & na/nr & na/nr \\
48    & \cite{diaz2002inno} & ICT   & meso  & descriptive & positive & support & na/nr & na/nr & na/nr \\
49    & \cite{dixon2020decline} & TFP-style & meso  & regression & negative & weak  & na/nr & no support & productivity; \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & income \\
50    & \cite{dodel2020perceptions} & robots & micro & regression & na/nr & support & na/nr & na/nr & na/nr \\
51    & \cite{dupaigne2009shock} & TFP-style & macro & regression & depends & na/nr & depends & na/nr & na/nr \\
52    & \cite{eden2018} & ICT   & macro & regression & na/nr & support & na/nr & na/nr & na/nr \\
53    & \cite{edler1994tech} & robots & meso  & other & weak  & support & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & (simulation) & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
54    & \cite{ergul2020tech} & TFP-style & macro & other & na/nr & support & na/nr & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & (simulation) & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\bottomrule
\end{tabular}


==> inputs/studies2.tex <==
\begin{tabular}{ll*{8}{c}}
\toprule
\multicolumn{2}{c}{Studies} & \multicolumn{3}{c}{Categories} & \multicolumn{5}{c}{Findings for technology effects on} \\
\midrule
\multicolumn{1}{p{2em}}{\#} & Authors \& year & Technology & Level of  & Empirical & Net   & Replacement & Reinstatement & \multicolumn{2}{c}{Real income} \\
\cmidrule{9-10}      & \multicolumn{1}{c}{} & group & analysis & methods & employment & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & finding & type \\
\midrule
55    & \cite{evangelista2012inno} & innovation & micro & regression & positive & depends & depends & na/nr & na/nr \\
56    & \cite{faber2020robot} & robots & regional & regression & na/nr & support & na/nr & na/nr & na/nr \\
57    & \cite{fagerberg1997tech} & other/indirect & regional & regression & positive & na/nr & support & support & output \\
58    & \cite{falk2015inno} & innovation & micro & regression & na/nr & depends & na/nr & na/nr & na/nr \\
59    & \cite{feldmann2013} & other/indirect & macro & regression & weak  & support & support & na/nr & na/nr \\
60    & \cite{flug2000} & other/indirect & macro & regression & depends & depends & na/nr & na/nr & na/nr \\
61    & \cite{fonseca2018polar} & ICT   & micro & regression & na/nr & support & weak  & na/nr & na/nr \\
62    & \cite{fort2018} & TFP-style & meso; & descriptive & depends & depends & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & micro & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
63    & \cite{fossen2021digital} & ICT   & micro & regression & na/nr & support & support & na/nr & na/nr \\
64    & \cite{fu2021} & robots & macro; & regression & positive & no support & na/nr & depends & productivity \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & regional & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
65    & \cite{fung2006} & ICT;  & micro & regression & positive & no support & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & innovation & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
66    & \cite{gaggl2017computer} & ICT   & micro & regression & depends & no support & support & na/nr & na/nr \\
67    & \cite{gallipoli2018it} & ICT   & macro & descriptive & depends & depends & support & na/nr & na/nr \\
68    & \cite{gardberg2020digit} & other/indirect & macro; & regression & negative & support & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & micro & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
69    & \cite{gentili2020machines} & robots & meso  & descriptive & positive & na/nr & support & na/nr & na/nr \\
70    & \cite{gera2001tech} & other/indirect & meso  & regression & na/nr & support & na/nr & na/nr & na/nr \\
71    & \cite{goaied2019} & ICT   & macro & regression & negative & support & no support & support & output \\
72    & \cite{graetz2018robots} & robots & meso  & regression & weak  & support & support & support & prices; \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & productivity; \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & income \\
73    & \cite{graham2000} & TFP-style & regional; & regression & depends & support & support & support & output \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & meso  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
74    & \cite{green2015} & other/indirect & macro & descriptive & depends & weak  & support & na/nr & na/nr \\
75    & \cite{gregory2001jobs} & TFP-style & meso  & descriptive & na/nr & support & na/nr & na/nr & na/nr \\
76    & \cite{grigoli2020automation} & other/indirect & macro; & regression & na/nr & support & na/nr & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & micro & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
77    & \cite{ho2008invest} & TFP-style; & meso  & regression & na/nr & support & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & other/indirect & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
78    & \cite{hoskins2000} & other/indirect & macro & regression & depends & support & support & na/nr & na/nr \\
79    & \cite{hoskins2002} & other/indirect & macro & regression & negative & support & na/nr & na/nr & na/nr \\
80    & \cite{huh2019} & TFP-style & macro & regression & negative & support & na/nr & na/nr & na/nr \\
81    & \cite{idris2021tech} & other/indirect & macro & regression & weak  & weak  & na/nr & na/nr & na/nr \\
82    & \cite{ivus2015broadband} & ICT   & regional & regression & depends & no support & support & na/nr & na/nr \\
83    & \cite{jerbashian2019autom} & ICT   & meso  & regression & depends & support & support & na/nr & na/nr \\
84    & \cite{jiang2019subst} & other/indirect & macro & regression & positive & na/nr & support & na/nr & na/nr \\
85    & \cite{jung2020tech} & robots & meso  & regression & negative & support & na/nr & support & productivity \\
86    & \cite{kaiser2001} & ICT   & micro & regression & depends & support & support & na/nr & na/nr \\
87    & \cite{karabarbounis2013lshare} & other/indirect & macro & regression & negative & na/nr & na/nr & na/nr & na/nr \\
88    & \cite{kim2020lshare} & TFP-style; & regional & regression & depends & support & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & other/indirect & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
89    & \cite{kristal2013capitalist} & ICT   & meso  & regression & depends & support & support & na/nr & na/nr \\
90    & \cite{kwon2015inno} & innovation & micro & regression & depends & depends & depends & na/nr & na/nr \\
91    & \cite{labaj2020automation} & robots & macro & regression & depends & support & support & na/nr & na/nr \\
92    & \cite{leigh2019robots} & robots & regional; & regression & positive & na/nr & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & meso  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
93    & \cite{luker1997employment} & ICT   & meso  & descriptive & positive & support & support & na/nr & na/nr \\
94    & \cite{madariaga2018employment} & other/indirect & macro & regression & depends & support  & support & na/nr & na/nr \\
95    & \cite{manning2004tech} & other/indirect & regional & regression & positive & support & na/nr & na/nr & other \\
96    & \cite{maurin2004skill} & ICT   & micro & regression & depends & weak  & support & na/nr & na/nr \\
97    & \cite{morrisonpaul2001tech} & ICT;  & meso  & regression & na/nr & support & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & other/indirect & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
98    & \cite{morrison1997} & ICT;  & meso  & regression & depends & support & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & other/indirect & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
99    & \cite{oesch2010} & other/indirect & macro & descriptive & depends & support & support & weak  & other \\
100   & \cite{omahony2021lshare} & ICT;  & macro; & regression & depends & depends & depends & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & other/indirect & meso  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
101   & \cite{oulton2002ict} & ICT   & macro & descriptive & na/nr & na/nr & na/nr & support & productivity \\
102   & \cite{padalino1997employment} & other/indirect & macro & regression & positive & support & support & support & output \\
103   & \cite{pantea2017ict} & ICT   & micro & regression & na/nr & no support & na/nr & na/nr & na/nr \\
104   & \cite{pellegrino2019rnd} & innovation & micro & regression & depends & depends & depends  & na/nr & na/nr \\
105   & \cite{peng2018it} & other/indirect & micro & regression & depends & support & na/nr & na/nr & na/nr \\
106   & \cite{piva2004change} & innovation & micro & regression & weak  & na/nr & weak  & na/nr & na/nr \\
107   & \cite{piva2005innovation} & innovation & micro & regression & weak  & na/nr & weak  & na/nr & na/nr \\
108   & \cite{raval2019micro} & other/indirect & micro & regression & positive & no support & support & na/nr & na/nr \\
109   & \cite{reijnders2018tech} & other/indirect & macro & regression & depends & support & support & na/nr & na/nr \\
110   & \cite{reshef2013tech} & other/indirect & macro & other & na/nr & support & support & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & (simulation) & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
111   & \cite{sala2018effects} & TFP-style & macro & regression & positive & no support & support & na/nr & na/nr \\
112   & \cite{samaniego2006tech} & other/indirect & macro & other & na/nr & na/nr & na/nr & no support & productivity \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & (simulation) & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
113   & \cite{samaniego2008tech} & other/indirect & macro & other & positive & na/nr & na/nr & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & (simulation) & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\bottomrule
\end{tabular}


==> inputs/studies3.tex <==
\begin{tabular}{ll*{8}{c}}
\toprule
\multicolumn{2}{c}{Studies} & \multicolumn{3}{c}{Categories} & \multicolumn{5}{c}{Findings for technology effects on} \\
\midrule
\multicolumn{1}{p{2em}}{\#} & Authors \& year & Technology & Level of  & Empirical & Net   & Replacement & Reinstatement & \multicolumn{2}{c}{Real income} \\
\cmidrule{9-10}      & \multicolumn{1}{c}{} & group & analysis & methods & employment & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & finding & type \\
\midrule
114   & \cite{sargent2000unempl} & other/indirect & macro & descriptive & depends & no support & na/nr & na/nr & na/nr \\
115   & \cite{scholl2020autom} & other/indirect & micro & regression & na/nr & no support & na/nr & na/nr & na/nr \\
116   & \cite{strohmaier2016ict} & ICT   & macro; & regression & na/nr & na/nr & na/nr & support & productivity \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & meso  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
117   & \cite{tether1998employment} & innovation & micro & descriptive & positive & na/nr & support & na/nr & na/nr \\
118   & \cite{vainiomaki1999tech} & other/indirect & meso  & descriptive & depends & support & support & na/nr & na/nr \\
119   & \cite{vanreenen1997inno} & innovation & micro & regression & depends & depends & depends & na/nr & na/nr \\
120   & \cite{vanroy2018tech} & other/indirect & micro & regression & positive & na/nr & support & na/nr & na/nr \\
121   & \cite{vivarelli1996inno} & innovation & micro & regression & na/nr & support & support & na/nr & na/nr \\
122   & \cite{vu2013ict} & ICT   & meso  & regression & na/nr & na/nr & na/nr & support & productivity; \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & output \\
123   & \cite{wemy2019lshare} & other/indirect & macro & regression & negative & support & na/nr & na/nr & na/nr \\
124   & \cite{whelan2009shocks} & TFP-style & macro & regression & negative & support & na/nr & na/nr & na/nr \\
125   & \cite{wolff2009computer} & ICT   & macro; & regression & na/nr & support & na/nr & na/nr & na/nr \\
      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & meso  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
126   & \cite{xiang2005} & innovation & meso  & regression & positive & na/nr & support & na/nr & na/nr \\
127   & \cite{yildirim2020} & other/indirect & macro & regression & positive & na/nr & support & na/nr & na/nr \\
\bottomrule
\end{tabular}

